CoCo Matrix: Taxonomy of Cognitive Contributions in Co-writing with Intelligent Agents

In recent years, there has been a growing interest in employing intelligent agents in writing. Previous work emphasizes the evaluation of the quality of end product-whether it was coherent and polished, overlooking the journey that led to the product, which is an invaluable dimension of the creative process. To understand how to recognize human efforts in co-writing with intelligent writing systems, we adapt Flower and Hayes' cognitive process theory of writing and propose CoCo Matrix, a two-dimensional taxonomy of entropy and information gain, to depict the new human-agent co-writing model. We define four quadrants and situate thirty-four published systems within the taxonomy. Our research found that low entropy and high information gain systems are under-explored, yet offer promising future directions in writing tasks that benefit from the agent's divergent planning and the human's focused translation. CoCo Matrix, not only categorizes different writing systems but also deepens our understanding of the cognitive processes in human-agent co-writing. By analyzing minimal changes in the writing process, CoCo Matrix serves as a proxy for the writer's mental model, allowing writers to reflect on their contributions. This reflection is facilitated through the measured metrics of information gain and entropy, which provide insights irrespective of the writing system used.

==> 04-dimensions.tex <==
\subsection{Dimensions of Human-AI Co-writing}
% define engagement by interfece options, writing goals 
% determine information gain & entropy is to measure the contribution 
Authors' writing goals profoundly shape idea organization and presentation. During human-AI co-writing, the UI Interface choice influences the interaction type. Notable interaction methods include: prompting \cite{dang2023choice},in-text editing \cite{du2022read}, conversation interaction, design Space interaction \cite{chung2022talebrush, zhang2023visar}.
%\textbf{Prompting}: Users provide a theme or prompt for the AI to base its content on. The AI generates a response, which users can then expand, refine, or edit to achieve the desired writing piece \cite{yuan2022wordcraft}.
%\textbf{In-Text Editing}: AI tools assist in the revision process by offering suggestions for grammar correction, content enhancement, and ensuring writing flow \cite{du2022read}.
%\textbf{Conversation interaction}: Users engage in a conversation with the AI, initiating discussions, posing questions, or making statements. The AI's responses aid in collaboratively creating content, as seen in platforms like ChatGPT.
%\textbf{Design Space Interaction}: Innovative interactions, such as line sketching for story trajectory control or visual argumentative structure creation, offer unique ways of collaborating with AI \cite{chung2022talebrush, zhang2023visar}.
These interaction methods reflect diverse approaches to human-AI co-writing, catering to various writing goals and phases, including planning, translation, and review. 
Adapting Flower's cognitive theory \cite{flower1981cognitive}, we propose using information gain and entropy to describe the flow of information between the writing process, changes in the task environment, and updates to the writer's long-term memory, as shown in Figure \ref{fig:updated cognitive process}. Information gain and entropy help understand writers' engagement in writing and reflect writers' intellectual contribution in co-writing with AI assistants. 
\tlcomment{need a lot more explanation/rationale}

\subsubsection{Entropy}
%SIMRET
Entropy, particularly in information theory, measures the uncertainty or randomness in data. It is often used to quantify the amount of information, surprise, or uncertainty in a series of symbols or actions~\cite{dai2013entropy}.
Entropy in information theory is defined as follows:
\[ H(X) = -\sum_{i=1}^{n} P(x_i) \log_b P(x_i) \]
where \( H(X) \) is the entropy of the random variable \( X \), \( P(x_i) \) represents the probability of each outcome \( x_i \), and the base of the logarithm \( b \) determines the unit of entropy.
Entropy in the context of the actual writing actions — such as planning, revising, and translating — can be understood as a measure of the degree of order or disorder in the creative process. In the planning phase, entropy is low. Writers typically start with a structured outline or a clear idea of what they want to write. This phase is characterized by organized thoughts and a coherent vision of the narrative or content. The low entropy here represents a high level of structure.

In the drafting phase of writing, entropy increases. This phase often involves exploring different narrative paths, character developments, and stylistic choices. The initial structure may give way to new ideas, leading to a state of higher unpredictability and creative exploration in serendipitous learning. This phase embodies the concept of entropy as the writer navigates through a more chaotic and less predictable creative process. The process of refining and revising a written draft, imposes order on the chaotic elements introduced during drafting, thus reducing entropy and moving towards a more structured written piece.
Entropy is a dynamic element in writing, fluctuating through different stages of the writing process. It represents the tension between order and chaos, structure and creativity, and is integral to the evolution of a piece from an initial idea to a polished work. 

\subsubsection{Information Gain}
%Ruyuan
In information theory and machine learning, information gain quantifies the information acquired about a random variable by observing another variable. It also denotes reduced information entropy (H) when transitioning from a prior state to a state where specific information is given.

\[ IG(T, a) = H(T) - H(T|a)\] where $H(T|a)$ is the conditional entropy of T given the value of attribute a. As we learn more about T (denoted as "$a$"), we decrease the uncertainty associated with $T$, which constitutes gaining information.

Applying information gain to the writing process enables the quantitative assessment of a writer's journey over time. It allows measuring the information contributed by the writer during prompting, revision, and content generation using AI writing tools.
Similar to entropy, information gain fluctuates throughout different stages of the writing process. During prompting and initial idea generation, writers contribute valuable information to shape the direction of the narrative or content. As the writing progresses and revisions occur, the AI tool may generate additional information, further refining the piece. In summary, information gain is a metric for evaluating the dynamic interaction between human writers and AI writing tools. It provides insights into how writers contribute to the writing process and how AI tools enhance writing.




